On Linking Level Segments

An increasingly common area of study in procedural content generation is the creation of level segments: short pieces that can be used to form larger levels. Previous work has used basic concatenation to form these larger levels. However, even if the segments themselves are completable and well-formed, concatenation can fail to produce levels that are completable and can cause broken in-game structures (e.g. malformed pipes in Mario). We show this with three tile-based games: a side-scrolling platformer, a vertical platformer, and a top-down roguelike. Additionally, we present a Markov chain and a tree search algorithm that finds a link between two level segments, which uses filters to ensure completability and unbroken in-game structures in the linked segments. We further show that these links work well for multi-segment levels. We find that this method reliably finds links between segments and is customizable to meet a designer's needs.

==> body-exag_draft.tex <==
%============================================================
\section{Introduction}

In the field of procedural content generation (PCG), a major focus of the research community is the creation of levels \cite{shaker2016procedural}. Approaches vary from  graph grammars \cite{hauck2020automatic} to machine learning \cite{summerville2018procedural} to reinforcement learning \cite{khalifa2020pcgrl} to behavior trees \cite{sarkar2021procedural} to search \cite{togelius2011search} and more. Work in the area of PCG, though, has done little to explore how generated levels, or parts of levels, can be successfully connected to form larger levels. We define success not only in terms of whether the connected level can be beaten but also in terms of the look and feel of the level. 

The simplest approach to combining generated level segments is to place them next to each other \cite{volz2018evolving}. More involved approaches can use the previous segment as input into a model to produce the next segment \cite{sarkar2020sequential}. Another approach is to require padding on either side of a generated level segment to guarantee a connection \cite{green2020mario}. Note, though, that each of these examples use \textit{Mario} where, as we will show, the lack of any additional connection between segments is likely to result in a playable level.

In this work, we explore an n-gram approach to generating \emph{linkers}: short pieces of a level that connect level segments. When two segments are linked together, the full level should be \emph{completable} (i.e. a player can get from the beginning to the end) and \emph{generable} (i.e. could have been generated by the model that created the segments). A resulting level is \emph{usable} if it is both completable and generable.

We use level segments generated by gram-elites \cite{biemer2021gram}, an approach based on MAP-Elites \cite{mouret2015illuminating} that uses n-grams to assemble slices (i.e. rows of columns) of training levels into segments with a variety of characteristics. We look at three games: \textit{Mario}, a horizontal platformer, \textit{Kid Icarus}, a vertical platformer, and \textit{DungeonGrams}, a top-down roguelike we developed. We compare the \emph{null} linker---concatenation of two segments---to other n-gram based linking methods. We examine the following results:

\begin{itemize}
\item Likelihood of finding a set of independent links for $k$ segments
\item Likelihood of the whole level---$k$ segments and $k-1$ independent links---being completable and usable
\item Length of n-gram based linkers and ability to match surrounding segments in terms of their characteristics (e.g. block density)
\end{itemize}


We find that for \textit{Mario} and \textit{DungeonGrams}, using a null linker is a little more likely to produce completable levels than n-gram based linking. But, in the case of \textit{Icarus}, using a null linker is less than half as likely to produce a completable level, especially as the number of level segments increases. We also find that chaining together segments that are independently linkable is very likely to result in an overall completable level. For all three games, completable levels made with the null linker are very unlikely to be generable by an n-gram and, consequently, do not meet our definition of usable. Lastly, it is possible to control the characteristics of linkers at the cost of increased length.



%============================================================
\section{Related Work}

This section is broken into two parts. First, we look at previous work that has combined vertical slices and tree search to generate levels. Second, we examine previous work that has combined level segments to form larger levels.

%------------------------------------------------------------
\subsection{N-Grams and Tree Search}

\textit{Mario} levels can be broken down from a grid to an ordered set of vertical slices \cite{dahlskog2014linear}. Dahlskog et al. use these vertical slices as input to an n-gram \cite{jurafsky2000speech} to generate levels. \cite{summerville2015mcmcts} expand on this by using the vertical slices as training data for a Markov chain where the output can be more than a single vertical slice but a set of them. They use Monte-Carlo tree search (MCTS) \cite{coulom2006efficient} to generate full levels. Unlike in n-gram generation where there are no guarantees as to what the n-gram will produce, the addition of tree search allows them to produce levels that are completeable, generable, and  matched to target behavioral characteristics.

%------------------------------------------------------------
\subsection{Using Level Segments}

\cite{sarkar2020sequential} use variational autoencoders (VAE) \cite{kingma2013auto} trained on levels with path information to generate level segments. The VAE was trained to encode a level segment and then use the encoding to predict the segment that follows. A level is generated by starting with one segment and then sequentially building new segments with the VAE. Meaning, the VAE is performing the role of generating segments sequentially in a way that they connect to each other.

\cite{volz2018evolving} trained a generative adversarial network (GAN) \cite{goodfellow2014generative} on a single \textit{Mario} level. Their innovation in the process was to search the latent space of the generative network with CMA-ES \cite{hansen2003reducing}. In one of their experiments, they tested forming larger levels of segments with increasing difficulty. This was accomplished by generating the level segments with a target difficulty and then placing them together.

\cite{green2020mario} start with a corpus of \textit{Mario} levels that have been generated with a required padding of two vertical slices of ground tiles on either side \cite{khalifa2019intentional}. The completable segments are placed together with padding to form larger levels. The best combination is found is by using FI-2Pop \cite{kimbrough2005introducing}. The combination of level segments and padding is feasible if it can be beaten. The sequence is further optimized by FI-2Pop based on a target mechanics sequence.
  
% \cite{hauck2020automatic} use the following pipeline: structure identification, structure matching, and level generation. The technical details of structure identification are out of scope for this work. However, an important stopping criteria for a structure identification is when it and another structure have overlap, which is the first criteria for structure matching. The second criteria is if the combination of the two structures is completable by an agent. If so, a link between the two is made. The end result of structure matching is a graph-grammar which is used in level generation. They found that levels generated with a minimum of 35 structures were $97\%$ likely to be playable from start to finish.

\cite{li2021ensemble} use an ensemble of Markov chain models to generate \textit{Mega Man} levels. They use a first-order Markov chain to model the direction (i.e. horizontal or vertical) of a set of rooms. They use two L-shape Markov chains \cite{snodgrass2014hierarchical} to generate the rooms, one for horizontal rooms and the other for vertical rooms. They place these rooms together and run a check to guarantee that a path from one to the other exists. If a valid path does not exist, they re-sample until two rooms with a connection are found.




%============================================================
\section{Approach}

Here we describe our approach. First, we give a brief overview of gram-elites, which we used to generate level segments. Next, we review the games used in this work. Finally, we discuss linking two segments together with a tree search on an n-gram and the types of linkers we generate.

%------------------------------------------------------------
\subsection{Gram-Elites}

Gram-elites \cite{biemer2021gram}, developed in prior work, is an extension to MAP-Elites \cite{mouret2015illuminating} that uses n-grams for population generation and the genetic operators mutation and crossover.  Like MAP-Elites, gram-elites uses behavioral characteristics to differentiate level segments. Gram-elites guarantees that all output segments are generable by an n-gram and optimizes segment completability. Consequently, we filter out resulting segments that are not completable by an agent.

When segments are modified by the genetic operations in gram-elites, a concept called \textit{connection} is used to connect parts of segments. This ensures that after an internal modification to a segment, the result will still be generable by an n-gram. This is accomplished with a breadth-first search through an n-gram from the $n-1$ slices before the modification (start prior) to the $n-1$ slices after the modification (end prior). %Such a path will always exist if there is a path from every prior to every other prior, which we ensured in the n-grams used in this work.



%------------------------------------------------------------
\subsection{Games}

Here we review the three games used to evaluate n-gram based linking. We briefly describe the behavioral characteristics, but more details can be found in \cite{biemer2021gram}. We also give details on n-gram training data and size, level size, and the agent used to evaluate completability. When evaluating completability, we pad the very beginning and very end of the slices being evaluated with a few slices, to have a place for the player to begin and end the level; these are omitted from figures.

\noindent
\textbf{Mario} is a horizontal platformer. We use behavioral characteristics linearity and leniency \cite{smith2010analyzing}. Linearity is based on the level’s fit to a line going through the highest points of each column. Leniency is calculated based on the number of gaps and enemies in a level. We use trigrams, training levels from the VGLC \cite{summerville2016vglc}, and segments are 25 slices long. We use a modified Summerville A* agent \cite{summerville2016vglc} to calculate the furthest point in the level that can be reached. 

\noindent
\textbf{Kid Icarus} is a vertical platformer. We use behavioral characteristics density and leniency. Density is the percent of solid blocks. Leniency is based on the existence of doors, moving platforms, and enemies. We use bi-grams, training levels from the VGLC \cite{summerville2016vglc}, and segments are 25 slices tall. We use a modified Summerville A* agent \cite{summerville2016vglc} to calculate the furthest point in the level that can be reached.
 
\noindent
\textbf{DungeonGrams} is a top-down rogue-like developed in previous work \cite{biemer2021gram}. The player has to progress left-to-right and hit switches to unlock a portal and then use it as an exit to beat a level. There are spikes and enemies that the player has to avoid while navigating a level. In particular, in this work, we extended \textit{DungeonGrams} to add a stamina mechanic. The player has a limited number of moves before they lose. The player can find food along the way to increase their stamina. This was done to make the game more challenging and make generating completable levels more difficult for the generator and linker.  

We use behavioral characteristics density and leniency. Density is the percent of solid blocks. Leniency is based on the existence of enemies, spikes, and switches. We use trigrams, along with training levels and a search-based agent created for the game. Segments are 15 slices long.


%------------------------------------------------------------
\subsection{Generating Linkers}

We use the n-gram connection approach from gram-elites to create linkers between two given segments.  This is done by a breadth-first search through the n-gram to connect the last slices of the starting segment (i.e. start prior) to the first slices of the end segment (i.e. end prior).

We also check the completability of the linked segments; that is, the combination of the start segment, linker, and end segment must be completable by an agent. Note that since we only use segments from gram-elites that can be completed, we are effectively testing that the linking of the two segments maintains this completability.  Additionally, in order to not generate unreasonably long linkers relative to segment size and improve performance, we limit the depth of the search to six.  It is possible that two given segments may not be linkable if there is no completable path found within that depth.

Since segments are generated by gram-elites, they have particular behavioral characteristics. We may want the linkers between them to have similar characteristics.  As a measure of this similarity, we can look at the root mean squared error (RMSE) between that linker's behavioral characteristics and the average of the behavioral characteristics of the segments it is linking.

Here we describe the types of linkers we generate:


\noindent
\textbf{Null}: This linker concatenates two segments (i.e. a linker of length zero). For the link to be classified as successful, the completability check must pass. Note that this type of linker may result in a level that has several problems. The new level may not be generable by an n-gram and, therefore, it may not visibly match the style of the game. Relatedly, the new level can violate tile constraints and, potentially, break player immersion, see Figure \ref{XfigureMalformedPipe}.


\noindent
\textbf{Shortest}: This type is the shortest (i.e. first) completable linker found by the depth-limited n-gram search. By searching the n-gram, these linkers, if found, are generable.

\noindent
\textbf{BC-match}: This type of linker uses an exhaustive, depth-limited n-gram search to find the completable linker with the lowest behavioral characteristic RMSE. Again, these linkers are generable.

\noindent
\textbf{BC-match-f}: In \textit{DungeonGrams}, food is a valuable resource.  This type of linker is the same as BC-match but also requires that the linker have food in it.  In-game, this could let the player refresh their stamina before proceeding to the next segment.  This type of linker is only used for \textit{DungeonGrams}, which also demonstrates the possibility of generating linkers using game-specific criteria.


%============================================================
\section{Evaluation}

\XFigureMarioLinkers
\XFigureIcarusLinkers
\XFigureGoodLink

\XFigureNullSuccess
\XfigureMalformedPipe

For each game, we ran gram-elites, using the behavioral characteristics described above, to generate a variety of segments. To explore the linking types, we wanted to determine: 1) how often are pairs of segments linkable; 2) when pairs of segments are independently linkable, are levels resulting from chaining them together completable and usable; and 3) how well do linkers match desired behavioral characteristics.

Linker types are tested by creating full levels that link together $k \in {2, 3, 4}$ segments together. For each $k$, we randomly select $k$ segments 1000 times and try to link them into a full level using each of the linker types.  Note that linkers are built independently (e.g. linking segments $A$, $B$, and $C$ will build a link between $A$ and $B$ that doesn't know about $C$ and another link between $B$ and $C$ that does not take into account $a$ and the associated link to $B$). We consider a level \textit{linkable} if each pair of segments is independently successful in linking. A linkable level is \textit{completable} if the entire resulting level can be completed by an agent. A completable level is \textit{usable} if it is \textit{generable} by the n-gram.

\XTABLELinksFound

Table \ref{XTABLELinksFound} shows information about the links found. For linkability, null linkers for \textit{Mario} and \textit{DungeonGrams}  were able to link segments the most often for all $k$. Although, \textit{DungeonGrams} levels were less linkable overall. We believe this is due to stamina restricting what is completable, and the null linker produces short levels. The null linker for \textit{Icarus} performs relatively poorly. We expect the verticality of the game requires linkers to add platforms to help make progress, see Figure \ref{XFigureIcarusLinkers}.  The shortest and BC-match linkers perform identically in terms of being able to link segments. In \textit{DungeonGrams}, the BC-match-f linkers were the least likely to be able to find a link, given their additional requirement of having food in the linker.


Figure \ref{XFigureMarioLinkers} shows a \textit{Mario} example where the null linker is not completable and the other linkers are; Figure \ref{XFigureIcarusLinkers} gives a similar example for \textit{Icarus}. Figure \ref{XFigureGoodLink} shows an example from \textit{DungeonGrams} where the addition of a link containing food makes a level completable. Figure \ref{XFigureNullSuccess} shows a \textit{Mario} example where the null linker is completable but the other linkers cannot find a link due to the depth limit. 

Looking at if linkable levels are completable, we see this is always the case for \textit{Icarus} and \textit{Mario}. For \textit{DungeonGrams}, every linker with $k \geq 3$ has cases where a linkable level is not a completable level. We expect that this is due, in part, to the agent starting with full stamina in the starting location when checking the independent linkability, but not necessarily having full stamina and/or being at that location when reaching the next segment in the full level. Since n-gram based linkers can increase the level length, it is likely that the agent runs into cases where it does not have enough stamina. In \textit{DungeonGrams}, BC-match-f linkers do appear to improve the likelihood of a linkable level being completable. Looking at $k=3$, BC-match-f linkers are the highest  at ${\sim}99\%$, while the other approaches are ${\sim}90\%$. For $k=4$, BC-match-f is improved to ${\sim}86\%$ from BC-match's $75\%$, which is similar to that of null (${\sim}85\%$) and shortest (${\sim}88\%$).

We see that when incorporating generability, which the null linker does not consider, the null linker has the fewest usable levels in all games when compared to the other approaches.



\XfigureBCSingular
\XFIGURELinkLengths
% \XfigureBC

Figure \ref{XfigureBCSingular} shows a violin plot on  how well linkers match desired behavioral characteristics, and Figure \ref{XFIGURELinkLengths} shows a violin plot for the length of the linkers. Null is not included in either figure since it does not have behavioral characteristics and its length is always zero. BC-match unsurprisingly has a lower RMSE than shortest for all three games since it optimizes for that metric. It also has longer linker lengths than shortest. For \textit{DungeonGrams}, BC-match-f has the longest linkers on average, and the RMSE ends up being slightly larger than BC-match.



%============================================================
\section{Discussion}

% sparsity in n-gram for DG not having enough food in it?


The null linking strategy for \textit{DungeonGrams} and \textit{Mario} outperforms n-gram based linking. In the case of \textit{Mario}, this is likely due to the simplicity of the game, and the depth limit on the search used by the linkers. In the case of \textit{DungeonGrams}, null linkers performs well due to two factors. First, the game's input levels do not include many high-density levels (i.e. it is likely for every segment to have an opening that lines up with an opening at the following segment). Second, a long link increases the likelihood that the player runs out of stamina before they can beat the level. This is also why shortest outperformed BC-match at $k=3$ and $k=4$. Further, the input levels are relatively sparse when it comes to placement of food which makes it unlikely, as seen by the smaller number of linkers found by BC-match-f, for a linker to include food.



For the most part, generability may only affect the visual style of the level. But \textit{Mario}, for example, has tiles that depend on others to look correct, specifically pipes. In Figure \ref{XfigureMalformedPipe}, we show an example of a level generated that is playable but has an incomplete pipe. As a result, we argue that the guarantee of generability is essential for designers who wish to maintain the style of their game when linking level segments; especially if their game includes structures that cover more than one tile.

\textit{Icarus} is the only game where n-gram linking appears to be mandatory for a combination of levels to be completable. As seen in the case of $k=4$, only two out of a thousand attempts of placing segments together were able to create a full level that can be beaten. Linking with n-grams is able to produce 150 usable levels, a $7400\%$ increase.

Overall, looking at the shortest and BC-match linkers it appears that it is possible to better match characteristics of neighboring segments at the cost of longer linkers.  In \textit{DungeonGrams}, BC-match-f shows that game-specific criteria can be included to improve the likelihood that linkable segments can chain into a completable level, but at the cost of fewer linkable segments overall.


%============================================================
\section{Conclusion}

% \item Likelihood of finding a set of independent links for $k$ segments
% \item Likelihood of the whole level---$k$ segments and $k-1$ independent links---being completable.
% \item Length of n-gram based linkers that result in usable levels.
% \item Ability of n-gram based linkers to match surrounding segments in terms of their characteristics (e.g. block density).

In this work, we present an approach to linking level segments with a depth-limited, exhaustive tree search on an n-gram. We compare this method to a shortest path and a null link strategy. We test all three on three games: \textit{Mario}, \textit{Kid Icarus}, and \textit{DungeonGrams}. We built a set of independent links for $k$ segments and found varying results for linkability and completability among the games. The null strategy found the most completable levels for \textit{DungeonGrams} and \textit{Mario}, and the exhaustive and shortest strategy both found the same amount of levels for \textit{Icarus}. Notably, the null strategy performed very poorly for \textit{Icarus}. 

Examining the length of the linkers and the RMSE between the linkers behavioral characteristics and the segments being connected, we found that the exhaustive search had the lowest error. This is not necessarily surprising as exhaustive does optimize for it. However, it could be important for player experience as the links found by exhaustive are more similar to the segments linked than the link found by shortest, although the exhaustive search finds longer. We have already shown an example of this problem with incomplete pipes in \textit{Mario}.  Overall, there can be a tradeoff between factors such as linker length, matching segment characteristics, and being generable by the n-gram that designers may want to consider (e.g. in \textit{Mario}, if a designer is less concerned with generability, then the null linker may be preferred, but if they are, they may prefer a different linker).

In this work we used n-grams to generate linkers, because that is what gram-elites use to generate segments.  However, we believe other models (e.g. wave function collapse \cite{Gumin_Wave_Function_Collapse_2016} or example-based model synthesis \cite{merrell2007example}) could be used to generate linkers if such a model was used to generate the segments.

\textit{DungeonGrams} also presents an interesting case for improving the likelihood that linkable levels will be completable. In this work we explored the game-specific requirement that linkers contain food to try to improve this.  There may be other  approaches to changing criteria for linkability, such as using a more limited or constrained agent (e.g. with less starting stamina in the case of \textit{DungeonGrams}) used to check completability of linkers than used for the full completability check.

We believe further exploration of n-gram structure and its input is warranted. We believe that one method to improve the approach is to either allow for back-off n-grams or to use a human-in-the-loop strategy that allows designers to build connections between distant priors to improve the expressiveness of the n-gram before running gram-elites and linking. To further extend this work, we want to use this as a method to connect gram-elites bins to form a directed graph. With this directed graph, we intend to build larger levels that can be tailored to individual players.


==> review_notes.tex <==
- [X] de-anonymize the GitHub links.
- [X] Make figure 4 prettier. (Waiting on reply from Seth on Slack.)
- [X] Transpose Table two

Review 1:

- [X] In the introduction, the authors introduce a definition for linker usability before defining a linker, which is a bit confusing. I suggest switching the order, and moving the usability definition to after the linker definition. 

Review 2: 

- [X]  The motivation of the introduction is very good, and it summarizes the major details of the approach and outcomes well.  The latter part and former part could be connected more strongly though, because I left the introduction wondering about impact.  If this technique can be applied atop *any* segment-based generator, I feel that is a strong and exciting claim (if I don't misunderstand the system's full operation and context).
- [ ] The related work is good, though I think the constraint-based approaches are underrepresented, especially WFC which has some connections to the probabilistic approach used here.
- [ ] It feels like there are many similarities between this work and the WFC approach of learning from witnessed transitions.  I am very curious to see a deeper exploration of this if space permits. (Waiting on reply from Seth on Slack.)
- [X] My understanding of "linking" evolved substantially during my read of the paper, so it may benefit from explicitly defining linking/linkers earlier on.
    --> I believe I addressed this in the introduction when I handled reviewer 1's first comment.
- [X] It should also be made clear early on that multiple link "slices" can appear in a row, and the search process figures out which and how many are needed.
- [X] The caption used for table 2 is way too long, move it to text.
- [X] Showing that this technique can lift a specific, known PCG system into a much more successful version of said system, and showing impact on level evaluation metrics, would be a much stronger evaluation.
- [X] I guess I find myself still wondering at the end of the paper what the role of gram-elites is in this work, and whether it may be distracting from the evaluation of the linking scheme.  The gram-elite part is not really evaluated, so I take it to be a baseline, but I don't know much about it as a baseline so it's not clear to me how to interpret the results.

- [ ] How could this generalize do levels that are more "square", i.e. without a strict horizontal or vertical bias?  and 
- [X] Is it possible to automatically synthesize the "custom" linking rows/columns, or do those necessarily require human intervention?

Reviewer 3: 

- [X] Missing text in the caption of Fig.8: "The agent in fails to reach"
- [X] In general the paper is well written, but there was one part that was less clear to me. Do the forward pass and the backward pass iterate over all slices of the level segment, or only the start/end of a segment? I would imagine the former makes more sense in fixing the level and Figure 2 also hints at this, but the text "When building a link (...) an incomplete structure?" seems to suggest the latter. Perhaps the authors could clarify this a bit more in the text?

Reviewer 4: 

- [X] Cite: Antonios Liapis. 2017. Multi-segment evolution of dungeon game levels. In Proceedings of the Genetic and Evolutionary Computation Conference (GECCO' 17). Association for Computing Machinery, New York, NY, USA, 203–210. DO
- [X] Cite:  D. Ashlock and C. McGuinness, "Automatic generation of fantasy role-playing modules," 2014 IEEE Conference on Computational Intelligence and Games, 2014, pp. 1-8, doi: 10.1109/CIG.2014.6932867.
- [X] While the generation of smaller segments and combining them is definitely an interesting approach, the introduction could have more motivation. For instance, presenting the tradeoffs between generating big levels and smaller segments would be beneficial. Why do we want to generate segments? Couldn't there be fine-grained control even if generating bigger levels? Likewise, an example would be beneficial so that the reader can grasp the idea.
- [X] There is little information about Gram-Elites. While not the main part of the paper, the authors should add information such as the behavior dimensions used when generating the levels.
- [X] While some more info on the behavior dimensions would be beneficial, I am curious to know how the linking affects the level in general. If the authors take the MAP-Elites generated grid and link neighbor by neighbor, how does this affect the final behavior feature of a level? For instance, if one combines segments with different lenient scores, what is the leniency of the final level? How could links force specific design constraints similar to the DG-Food? Discussing a bit more about that would be great and beneficial.
- [UWC] Comparison with other methods rather than concatenation would have been beneficial to support the approach further. Then it would be much more appreciable the strengths of the approach since it clearly outperforms concatenation. ---> What other methods?
- [X] The definition of linking columns is unclear. Are these defined by designers and are completely unrelated to the game? How are they generated/used by Gram-Elites?
- [X] Section IV-b, figure II should be changed to table II.

X - done
UWC - unaddressed with cause
